Obstacle-aware Waypoint Generation for Long-range Guidance of Deep-Reinforcement-Learning-based Navigation Approaches

Navigation of mobile robots within crowded environments is an essential task in various use cases, such as delivery, health care, or logistics. Deep Reinforcement Learning (DRL) emerged as an alternative method to replace overly conservative approaches and promises more efficient and flexible navigation. However, Deep Reinforcement Learning is limited to local navigation due to its myopic nature. Previous research works proposed various ways to combine Deep Reinforcement Learning with conventional methods but a common problem is the complexity of highly dynamic environments due to the unpredictability of humans and other objects within the environment. In this paper, we propose a hierarchical waypoint generator, which considers moving obstacles and thus generates safer and more robust waypoints for Deep-Reinforcement-Learning-based local planners. Therefore, we utilize Delaunay Triangulation to encode obstacles and incorporate an extended hybrid A-Star approach to efficiently search for an optimal solution in the time-state space. We compared our waypoint generator against two baseline approaches and outperform them in terms of safety, efficiency, and robustness.

==> ieeeconf/content/acknowledgment.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex



==> ieeeconf/content/keywords.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex


%\begin{IEEEkeywords}
%	Virtual Reality and Interfaces, Localization, Object Detection, Computer Vision for Other %Robotic Applications, AI-Based Methods
%\end{IEEEkeywords}

==> ieeeconf/content/title.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex

%\title{A robust pose estimator for articualted robots using monocular cameras and Deep-Learning-based keypoint detection\\
%	}
%	\thanks{Identify applicable funding agency here. If none, delete this.}
%}
\title{\LARGE \bf
Towards Augmented Reality Simulation in Robotics - Facing Barriers of Industrial Applicability
}

\author{Jens Lambrecht$^{1}$, Linh Kästner$^{1}$, Jan Guhl$^{2}$ and J\"org Kr\"uger$^{2}$% <-this % stops a space% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Jens Lambrecht and Linh Kästner are with the Chair Industry Grade Networks and Clouds, Faculty of Electrical Engineering and Computer Science,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small lambrecht@tu-berlin.de}}%
\thanks{$^{2}$Jan Guhl and J\"org Kr\"uger are with the Chair Industrial Automation Technology, Faculty of Mechanical Engineering and Transport Systems,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small guhl@iat.tu-berlin.de}}%        
}


%\author{
%	\IEEEauthorblockN{Jens Lambrecht}
%	\IEEEauthorblockA{\textit{Chair Industry Grade Networks and Clouds} \\
%		\textit{Technische Universität Berlin}\\
%		Berlin, Germany \\
%		lambrecht@tu-berlin.de}
%}

\maketitle
